Rethinking BPS: A Utility-Based Evaluation Framework

Business process simulation (BPS) is a key tool for analyzing and optimizing organizational workflows, supporting decision-making by estimating the impact of process changes. The reliability of such estimates depends on the ability of a BPS model to accurately mimic the process under analysis, making rigorous accuracy evaluation essential. However, the state-of-the-art approach to evaluating BPS models has two key limitations. First, it treats simulation as a forecasting problem, testing whether models can predict unseen future events. This fails to assess how well a model captures the as-is process, particularly when process behavior changes from train to test period. Thus, it becomes difficult to determine whether poor results stem from an inaccurate model or the inherent complexity of the data, such as unpredictable drift. Second, the evaluation approach strongly relies on Earth Mover's Distance-based metrics, which can obscure temporal patterns and thus yield misleading conclusions about simulation quality. To address these issues, we propose a novel framework that evaluates simulation quality based on its ability to generate representative process behavior. Instead of comparing simulated logs to future real-world executions, we evaluate whether predictive process monitoring models trained on simulated data perform comparably to those trained on real data for downstream analysis tasks. Empirical results show that our framework not only helps identify sources of discrepancies but also distinguishes between model accuracy and data complexity, offering a more meaningful way to assess BPS quality.

==> Tables/drift_results_new.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{12pt} % Adjust column spacing
    \caption{Comparison of different versions of the Loan Application process using our new framework for the evaluation (NPP, NWP, RTP in minutes).}
    \begin{tabular}{lrrrrr}
        \toprule
         & NAP & NRP & NPP & NWP & RTP \\
        \midrule
        Original-real & 0.79 & 0.83 & 86.4 & 14.5 & 216.0  \\
        Original-sim & 0.78 & 0.82 & 86.1 & 14.9 & 217.5  \\ 
        \midrule
        Drift-real & 0.83 & 0.39 & 83.2 & 259.2 & 806.4  \\
        Drift-sim & 0.82 & 0.37 & 84.9 & 261.1 & 805.1  \\
        \bottomrule
    \end{tabular}%
    \label{tab:results_drift_new}
\end{table}




==> Tables/results_LSTM.tex <==
\begin{table}[htbp]
    \centering
    \caption{Performance of LSTM model on real and simulated data. Each table entry shows the average performance over 10 runs, with the standard deviation in parentheses.}
    \begin{tabular}{clrrrrr}
        \toprule
        Log & Data & NAP & NRP & NPP(min) & NWP(hour) & RTP(day) \\
        \midrule
        \multirow{4}{*}{\rotatebox{90}{P2P}} & real & 0.84 (0.03) & 0.83 (0.01) & 70.24 (15.51) & 63.87 (0.72) & 20.10 (1.05) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.04 (0.00) & 0.07 (0.00) & 16.04 (0.00) & \textbf{1.09} (0.00) & \textbf{0.08} (0.00)\\
        & DSim & 0.12 (0.02) & NA & 21.44 (14.28) & 5.39 (5.80) & 7.39 (15.6) \\
        & ASim & \textbf{0.00} (0.02) & \textbf{0.04} (0.01) & \textbf{16.00} (7.94) & 2.04 (1.29) & 4.44 (6.78) \\   
        \midrule
        \multirow{4}{*}{\rotatebox{90}{C.1000}} & real & 0.71 (0.02) & 0.39 (0.00) & 21.23 (0.06) & 0.25 (0.00) & 0.41 (0.05) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.13 (0.01) & \textbf{0.00} (0.00) & 0.69 (0.47) & 1.09 (0.25) & 3.34 (2.52) \\
        & DSim & 0.48 (0.01) & NA & 5.67 (4.58) & 0.16 (0.07) & 0.04 (0.08) \\
        & ASim & \textbf{0.01} (0.02) & \textbf{0.00} (0.00) & \textbf{0.03} (0.04) & \textbf{0.02} (0.02) & \textbf{0.02} (0.06) \\        
        \midrule
        \multirow{4}{*}{\rotatebox{90}{C.2000}} & real &  0.71 (0.02) & 0.39 (0.00) & 21.44 (0.18) & 0.21 (0.00) & 0.38 (0.06) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.12 (0.01) & \textbf{0.00} (0.00) & 0.67 (0.31) & 1.47 (0.42) &  2.04 (2.41)\\
        & DSim & 0.50 (0.01) & NA & 3.29 (3.23) & 0.30 (0.09) & 1.65 (2.70) \\
        & ASim & \textbf{0.01} (0.03) & \textbf{0.00} (0.00) & \textbf{0.08} (0.09) & \textbf{0.01} (0.01) &  \textbf{0.02} (0.04)\\       
        \midrule        
        \multirow{4}{*}{\rotatebox{90}{CVS}} & real & 0.80 (0.03) & 0.94 (0.03) & 3.21 (0.06) & 25.36 (0.01) & 4.71 (0.01) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.30 (0.01) & 0.54 (0.08) & \textbf{0.00} (0.06) & 1.69 (0.24) & 2.02 (0.22) \\
        & DSim & 0.09 (0.01) & NA & 0.04 (0.02) & 29.89 (9.28) & 3.93 (2.57) \\
        & ASim & \textbf{0.02} (0.00) & \textbf{0.01} (0.00) & 0.06 (0.00) & \textbf{0.12} (0.06) & \textbf{0.10} (0.05) \\
        \midrule
        \multirow{4}{*}{\rotatebox{90}{Production}} & real & 0.54 (0.02) & 0.59 (0.02) & 120.00 (0.38) & 9.32 (0.29) &  5.75 (3.39)\\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.11 (0.03) & \textbf{0.14} (0.01) & 24.85 (10.37) & 41.50 (2.76) &  \textbf{0.05} (4.56)\\
        & DSim & 0.43 (0.07) & NA & \textbf{12.30} (6.06) & \textbf{9.21} (1.54) & 182.1 (112.90) \\
        & ASim & \textbf{0.00} (0.02) & 0.21 (0.07) & 27.87 (5.33) & 36.82 (2.95) & 2.93 (0.50) \\
        \midrule
        \multirow{4}{*}{\rotatebox{90}{CDM}} & real & 0.75 (0.02) & 0.68 (0.04) & 4.25 (0.13) & 12.31 (0.20) & 2.20 (0.02)\\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.27 (0.06) & 0.27 (0.04) & 0.49 (0.70) & 1.60 (1.00) & 0.11 (0.20) \\
        & DSim & 0.39 (0.08) & NA & 0.21 (0.18) & \textbf{0.10} (0.12) & \textbf{0.01} (0.02) \\
        & ASim & \textbf{0.13} (0.03) & \textbf{0.20} (0.07) & \textbf{0.04} (0.08) & 0.11 (0.06) & 0.01 (0.01) \\
        \midrule
        \multirow{4}{*}{\rotatebox{90}{BPI12W}} & real & 0.59 (0.06) & 0.75 (0.00) & 8.63 (0.13) & 26.53 (0.13) & 6.42 (0.94) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.38 (0.00) & \textbf{0.00} (0.00) & 0.21 (0.00) & 0.04 (0.00) & 0.20 (0.00) \\
        & DSim & 0.41 (0.02) & NA & 0.10 (0.05) & 0.05 (0.01) & \textbf{0.18} (0.03) \\
        & ASim & \textbf{0.02} (0.01) & \textbf{0.00} (0.00) & \textbf{0.04} (0.10) & \textbf{0.00} (0.11) & 0.21 (1.78) \\
        \midrule
        \multirow{4}{*}{\rotatebox{90}{BPI17W}} & real & 0.54 (0.01) & 0.88 (0.00) & 6.10 (0.55) & 33.01 (0.15) & 6.61 (0.40) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.23 (0.00) & 0.35 (0.00) & \textbf{0.56} (0.00) & 0.12 (0.00) & 0.68 (0.00) \\
        & DSim & 0.19 (0.02) & NA & 3.46 (3.66) & 0.10 (0.04) & 0.62 (0.06) \\
        & ASim & \textbf{0.08} (0.09) & \textbf{0.00} (0.00) & 1.70 (2.50) & \textbf{0.00} (0.15) & \textbf{0.25} (0.36) \\ 
        \bottomrule
    \end{tabular}
    \label{tab:results_LSTM}
\end{table}

==> Tables/results_Trans.tex <==
\begin{table}[htbp]
    \centering
    \caption{Performance of Transformer model on real and simulated data. Each table entry shows the average performance over 10 runs, with the standard deviation in parentheses.}
    \begin{tabular}{clrrrrr}
        \toprule
        Log & Data & NAP & NRP & NPP(min) & NWP(hour) & RTP(day) \\
        \midrule
        \multirow{4}{*}{\rotatebox{90}{P2P}} & real & 0.85 (0.01) & 0.88 (0.01) & 63.97 (3.26) & 61.88 (0.79) & 15.50 (0.22) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.02 (0.00) & \textbf{0.66} (0.00) & 114.22 (0.00) & \textbf{5.80} (0.00) & 2.96 (0.00) \\
        & DSim & 0.15 (0.03) & NA & 81.48 (89.20) & 6.86 (3.28) & 5.91 (4.05)\\
        & ASim & \textbf{0.00} (0.02) & \textbf{0.66} (0.04) & \textbf{17.21} (2.81) & 17.45 (3.84) & \textbf{1.66} (1.06) \\ 
        \midrule
        \multirow{4}{*}{\rotatebox{90}{C.1000}} & real & 0.74 (0.00) & 0.49 (0.01) & 17.06 (0.23) & 0.31 (0.01) & 0.36 (0.00) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.32 (0.02) & \textbf{0.12} (0.03) & \textbf{4.97} (034) & 3.05 (0.54) & 3.72 (0.44)\\
        & DSim & 0.55 (0.06) & NA & 7.22 (1.11) & \textbf{0.21} (0.01) & \textbf{0.10} (0.03)\\
        & ASim & \textbf{0.26} (0.02) & 0.18 (0.03) & 5.27 (0.56) & 0.37 (0.08) & 0.32 (0.07) \\
        \midrule
        \multirow{4}{*}{\rotatebox{90}{C.2000}} & real & 0.74 (0.00) & 0.54 (0.01) & 17.16 (0.41) & 0.28 (0.01) & 0.31 (0.01) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.28 (0.02) & \textbf{0.13} (0.05) & 4.98 (1.15) & 2.33 (0.35) & 3.11 (0.36)\\
        & DSim & 0.56 (0.05) & NA & 8.21 (1.16) & 0.38 (0.06) & \textbf{0.06} (0.04)\\
        & ASim & \textbf{0.19} (0.02) & 0.16 (0.13) & \textbf{4.89} (0.45) & \textbf{0.30} (0.07) & 0.21 (0.04) \\ 
        \midrule        
        \multirow{4}{*}{\rotatebox{90}{CVS}} & real & 0.72 (0.00) & 0.65 (0.00) & 3.32 (0.14) & 15.27 (0.50) & 1.61 (0.09) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.23 (0.01) & 0.65 (0.00) & 0.57 (0.33) & \textbf{27.57} (3.33) & 32.19 (1.88) \\
        & DSim & 0.19 (0.02) & NA & 0.61 (0.42) & 33.78 (10.22) & 15.82 (1.42)\\
        & ASim & \textbf{0.07} (0.01) & \textbf{0.06 (0.03)} & \textbf{0.12} (0.02) & 28.21 (4.82) & \textbf{1.18} (0.01) \\
        \midrule
        \multirow{4}{*}{\rotatebox{90}{Production}} & real & 0.59 (0.02) & 0.40 (0.04) & 121.66 (3.44) & 15.58 (1.69) & 10.61 (0.83) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.56 (0.02) & 0.31 (0.04) & 44.64 (53.96) & 12.73 (19.05) &  3.72 (20.12)\\
        & DSim & 0.48 (0.06) & NA & 12.11 (7.43) & 7.28 (1.21) & \textbf{0.05} (4.80)\\
        & ASim & \textbf{0.04} (0.02) & \textbf{0.01} (0.04) & \textbf{5.50} (2.70) & \textbf{5.06} (0.11) & 4.85 (0.99) \\
        \midrule 
        \multirow{4}{*}{\rotatebox{90}{CDM}} & real & 0.72 (0.00) & 0.55 (0.04) & 9.55 (0.83) & 8.58 (0.77) &  3.62 (0.13)\\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & \textbf{0.16} (0.04) & \textbf{0.31} (0.13) & 2.00 (1.22) & 25.61 (3.50) & 10.65 (0.60)\\
        & DSim & 0.51 (0.07) & NA & \textbf{0.46} (0.83) & 10.36 (1.39) & \textbf{0.64} (0.26)\\
        & ASim & 0.17 (0.02) & 0.48 (0.15) & 0.48 (2.03) & \textbf{6.17} (0.23) & 1.44 (0.02) \\   
        \midrule
        \multirow{4}{*}{\rotatebox{90}{BPI12W}} & real & 0.76 (0.00) & 0.86 (0.00) & 9.00 (0.20) & 29.59 (0.30) & 4.81 (0.10) \\
        \noalign{\vskip 1mm}
        \cdashline{2-7}
        \noalign{\vskip 1mm}
        & Simod & 0.48 (0.00) & 0.02 (0.00) & \textbf{0.31} (0.00) & 17.50 (0.00) & 0.65 (0.00) \\
        & DSim & 0.47 (0.02) & NA & 1.90 (0.70) & 4.45 (1.50) & 2.08 (0.36)\\
        & ASim & \textbf{0.00} (0.01) & \textbf{0.01} (0.00) & 0.50 (0.09) & \textbf{0.38} (0.21) & \textbf{0.18} (0.04) \\        
        \midrule
        \multirow{4}{*}{\rotatebox{90}{BPI17W}} & real & 0.62 (0.01) & 0.99 (0.00) & 6.14 (0.26) & 33.23 (0.43) & 5.80 (0.06) \\ 
        \noalign{\vskip 1mm}
        \cdashline{2-7}   
        \noalign{\vskip 1mm}
        & Simod & 0.20 (0.00) & \textbf{0.00} (0.00) & 0.25 (0.00) & 9.48 (0.00) & \textbf{0.70} (0.00) \\
        & DSim & 0.29 (0.09) & NA & 0.07 (0.22) & 21.95 (12.02) & 8.08 (2.83)\\
        & ASim & \textbf{0.12} (0.14) & 0.16 (0.14) & \textbf{0.06} (0.08) & \textbf{9.22} (7.19) & 3.10 (4.28)\\
        \bottomrule
    \end{tabular}
    \label{tab:results_transformer}
\end{table}

==> Tables/synthetic_KPIs.tex <==
\begin{table}[ht]
    \centering
    \caption{Average Process Metrics by Dataset (avg ± std)}
    \label{tab:process-metrics-std}
    \begin{tabular}{lcccc}
        \toprule
        Dataset & Cycle Time (hrs) & Duration (min) & Waiting (min) & Arrival (min) \\
        \midrule
        ground\_truth\_800   & 10.18 $\pm$ 16.20 & 95.88 $\pm$ 423.68  & 3.85 $\pm$ 95.97   & 30.00 $\pm$ 0.00 \\
        seq\_800           & 12.80 $\pm$ 17.31 & 96.46 $\pm$ 417.03  & 7.26 $\pm$ 120.16  & 30.00 $\pm$ 0.00 \\
        seq\_gat\_800      & 409.20 $\pm$ 510.78 & 101.09 $\pm$ 430.53 & 2616.44 $\pm$ 12498.73 & 30.00 $\pm$ 0.00 \\
        resource\_cont\_800  & 50.78 $\pm$ 30.42 & 95.16 $\pm$ 422.59  & 356.87 $\pm$ 979.25 & 29.99 $\pm$ 1.90 \\
        extraneous\_800    & 28.57 $\pm$ 23.50 & 132.45 $\pm$ 506.96 & 128.35 $\pm$ 477.47 & 30.00 $\pm$ 0.00 \\
        durations\_800     & 22.88 $\pm$ 22.38 & 184.29 $\pm$ 578.33 & 15.29 $\pm$ 174.35 & 30.00 $\pm$ 2.06 \\
        calendars\_800     & 9.67 $\pm$ 15.43  & 89.61 $\pm$ 391.79  & 4.83 $\pm$ 101.62  & 30.00 $\pm$ 0.00 \\
        arrivals\_800      & 10.18 $\pm$ 16.37 & 91.32 $\pm$ 408.15  & 8.80 $\pm$ 140.42  & 28.74 $\pm$ 29.04 \\
        \bottomrule
    \end{tabular}
\end{table}



==> Tables/temp.tex <==
\begin{table}[htbp]
    \centering
    \caption{Performance of predictive models on real and simulated data. LSTM and Transformer models are denoted by L and T in the column: "M". Each table entry shows the average performance over 10 runs, with the standard deviation in parentheses.}
    \begin{tabular}{cclrrrrr}
        \toprule
        Log & M & Data & NAP & NRP & NPP(min) & NWP(hour) & RTP(day) \\
        \midrule
        \multirow{8}{*}{\rotatebox{90}{P2P}} & L & real & 0.84 (0.03) & 0.83 (0.01) & 70.24 (15.51) & 63.87 (0.72) & 20.10 (1.05) \\
        & T & real & 0.85 (0.01) & 0.88 (0.01) & 63.97 (3.26) & 61.88 (0.79) & 15.50 (0.22) \\
        \cdashline{2-8}
        & L & Simod & -0.04 (0.00) & -0.07 (0.00) & +16.04 (0.00) & \textbf{+1.09} (0.00) & \textbf{-0.08} (0.00)\\
        & L & DSim & -0.12 (0.02) & NA & +21.44 (14.28) & +5.39 (5.80) & +7.39 (15.6) \\
        & L & ASim & \textbf{0.00} (0.02) & \textbf{-0.04} (0.01) & \textbf{+16.00} (7.94) & +2.04 (1.29) & +4.44 (6.78) \\
        & T & Simod & -0.02 (0.00) & \textbf{-0.66} (0.00) & +114.22 (0.00) & \textbf{+5.80} (0.00) & +2.96 (0.00) \\
         & T & DSim & -0.15 (0.03) & NA & +81.48 (89.20) & +6.86 (3.28) & +5.91 (4.05)\\
        & T & ASim & \textbf{0.00} (0.02) & \textbf{-0.66} (0.04) & \textbf{-17.21} (2.81) & +17.45 (3.84) & \textbf{+1.66} (1.06) \\     
        \midrule
        \multirow{8}{*}{\rotatebox{90}{Confidential 1000}} & L & real & 0.71 (0.02) & 0.39 (0.00) & 21.23 (0.06) & 0.25 (0.00) & 0.41 (0.05) \\
        & T & real & 0.74 (0.00) & 0.49 (0.01) & 17.06 (0.23) & 0.31 (0.01) & 0.36 (0.00) \\
        \cdashline{2-8}
        & L & Simod & -0.13 (0.01) & \textbf{0.00} (0.00) & +0.69 (0.47) & +1.09 (0.25) & +3.34 (2.52) \\
        & L & DSim & -0.48 (0.01) & NA & +5.67 (4.58) & +0.16 (0.07) & +0.04 (0.08) \\
        & L & ASim & \textbf{-0.01} (0.02) & \textbf{0.00} (0.00) & \textbf{-0.03} (0.04) & \textbf{+0.02} (0.02) & \textbf{+0.02} (0.06) \\
        & T & Simod & -0.32 (0.02) & \textbf{-0.12} (0.03) & \textbf{+4.97} (034) & +3.05 (0.54) & +3.72 (0.44)\\
        & T & DSim & -0.55 (0.06) & NA & +7.22 (1.11) & \textbf{+0.21} (0.01) & \textbf{+0.10} (0.03)\\
        & T & ASim & \textbf{-0.26} (0.02) & -0.18 (0.03) & +5.27 (0.56) & +0.37 (0.08) & +0.32 (0.07) \\
        \midrule
        \multirow{8}{*}{\rotatebox{90}{Confidential 2000}} & L & real &  0.71 (0.02) & 0.39 (0.00) & 21.44 (0.18) & 0.21 (0.00) & 0.38 (0.06) \\
        & T & real & 0.74 (0.00) & 0.54 (0.01) & 17.16 (0.41) & 0.28 (0.01) & 0.31 (0.01) \\
        \cdashline{2-8}
        & L & Simod & -0.12 (0.01) & \textbf{0.00} (0.00) & +0.67 (0.31) & +1.47 (0.42) &  +2.04 (2.41)\\
        & L & DSim & -0.50 (0.01) & NA & +3.29 (3.23) & +0.30 (0.09) & +1.65 (2.70) \\
        & L & ASim & \textbf{-0.01} (0.03) & \textbf{0.00} (0.00) & \textbf{-0.08} (0.09) & \textbf{+0.01} (0.01) &  \textbf{-0.02} (0.04)\\
        & T & Simod & -0.28 (0.02) & \textbf{-0.13} (0.05) & +4.98 (1.15) & +2.33 (0.35) & +3.11 (0.36)\\
        & T & DSim & -0.56 (0.05) & NA & +8.21 (1.16) & +0.38 (0.06) & \textbf{+0.06} (0.04)\\
        & T & ASim & \textbf{-0.19} (0.02) & -0.16 (0.13) & \textbf{+4.89} (0.45) & \textbf{+0.30} (0.07) & +0.21 (0.04) \\        
        \midrule
        \multirow{8}{*}{\rotatebox{90}{CVS}} & L & real & 0.80 (0.03) & 0.94 (0.03) & 3.21 (0.06) & 25.36 (0.01) & 4.71 (0.01) \\
        & T & real & 0.72 (0.00) &  & 3.32 (0.14) & 15.27 (0.50) &  \\
        \cdashline{2-8}
        & L & Simod & -0.30 (0.01) & -0.54 (0.08) & \textbf{0.00} (0.06) & +1.69 (0.24) & -2.02 (0.22) \\
        & L & DSim & -0.09 (0.01) & NA & -0.04 (0.02) & +29.89 (9.28) & +3.93 (2.57) \\
        & L & ASim & \textbf{-0.02} (0.00) & \textbf{+0.01} (0.00) & -0.06 (0.00) & \textbf{+0.12} (0.06) & \textbf{-0.10} (0.05) \\
        & T & Simod & -0.23 (0.01) &  & +0.57 (0.33) & \textbf{+27.57} (3.33) &  \\
        & T & DSim & -0.19 (0.02) & NA & +0.61 (0.42) & +33.78 (10.22) & \\
        & T & ASim & \textbf{-0.07} (0.01) &  & \textbf{-0.12} (0.02) & +28.21 (4.82) &  \\
        \bottomrule
    \end{tabular}
    \label{tab:results_synth}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Performance of predictive models on real and simulated data for event logs. LSTM and Transformer models are denoted by L and T in the column: "M". Each table entry shows the average performance over 10 runs, with the standard deviation in parentheses.}
    \begin{tabular}{cclrrrrr}
        \toprule
        Log & M & Data & NAP & NRP & NPP(min) & NWP(hour) & RTP(day) \\
        \midrule
        \multirow{8}{*}{\rotatebox{90}{Production}} & L & real & 0.54 (0.02) & 0.59 (0.02) & 120.00 (0.38) & 9.32 (0.29) &  5.75 (3.39)\\
        & T & real & 0.59 (0.02) & 0.40 (0.04) & 121.66 (3.44) & 15.58 (1.69) & 10.61 (0.83) \\
        \cdashline{2-8}
        & L & Simod & -0.11 (0.03) & \textbf{-0.14} (0.01) & +24.85 (10.37) & +41.50 (2.76) &  \textbf{-0.05} (4.56)\\
        & L & DSim & -0.43 (0.07) & NA & \textbf{+12.30} (6.06) & \textbf{+9.21} (1.54) & +182.1 (112.90) \\
        & L & ASim & \textbf{0.00} (0.02) & -0.21 (0.07) & -27.87 (5.33) & +36.82 (2.95) & -2.93 (0.50) \\
        & T & Simod & -0.56 (0.02) & -0.31 (0.04) & +44.64 (53.96) & +12.73 (19.05) &  +3.72 (20.12)\\
        & T & DSim & -0.48 (0.06) & NA & +12.11 (7.43) & +7.28 (1.21) & \textbf{+0.05} (4.80)\\
        & T & ASim & \textbf{-0.04} (0.02) & \textbf{+0.01} (0.04) & \textbf{-5.50} (2.70) & \textbf{-5.06} (0.11) & -4.85 (0.99) \\
        \midrule 
        \multirow{8}{*}{\rotatebox{90}{CDM}} & L & real & 0.75 (0.02) & 0.68 (0.04) & 4.25 (0.13) & 12.31 (0.20) & 2.20 (0.02)\\
        & T & real & 0.72 (0.00) & 0.55 (0.04) & 9.55 (0.83) & 8.58 (0.77) &  3.62 (0.13)\\
        \cdashline{2-8}
        & L & Simod & -0.27 (0.06) & -0.27 (0.04) & +0.49 (0.70) & +1.60 (1.00) & +0.11 (0.20) \\
        & L & DSim & -0.39 (0.08) & NA & +0.21 (0.18) & \textbf{+0.10} (0.12) & \textbf{-0.01} (0.02) \\
        & L & ASim & \textbf{-0.13} (0.03) & \textbf{-0.20} (0.07) & \textbf{-0.04} (0.08) & -0.11 (0.06) & +0.01 (0.01) \\
        & T & Simod & \textbf{-0.16} (0.04) & \textbf{-0.31} (0.13) & +2.00 (1.22) & +25.61 (3.50) & +10.65 (0.60)\\
        & T & DSim & -0.51 (0.07) & NA & \textbf{-0.46} (0.83) & +10.36 (1.39) & \textbf{-0.64} (0.26)\\
        & T & ASim & -0.17 (0.02) & -0.48 (0.15) & +0.48 (2.03) & \textbf{+6.17} (0.23) & -1.44 (0.02) \\
        \midrule
        \multirow{8}{*}{\rotatebox{90}{BPI12W}} & L & real & 0.59 (0.06) & 0.75 (0.00) & 8.63 (0.13) & 26.53 (0.13) & 6.42 (0.94) \\
        & T & real & 0.76 (0.00) & 0.86 (0.00) &  &  & 4.81 (0.10) \\
        \cdashline{2-8}
        & L & Simod & -0.38 (0.00) & \textbf{0.00} (0.00) & +0.21 (0.00) & +0.04 (0.00) & +0.20 (0.00) \\
        & L & DSim & -0.41 (0.02) & NA & -0.10 (0.05) & +0.05 (0.01) & \textbf{+0.18} (0.03) \\
        & L & ASim & \textbf{+0.02} (0.01) & \textbf{0.00} (0.00) & \textbf{-0.04} (0.10) & \textbf{0.00} (0.11) & +0.21 (1.78) \\
        & T & Simod & -0.48 (0.00) & -0.02 (0.00) &  &  & +0.65 (0.00) \\
        & T & DSim & -0.47 (0.02) & NA &  &  & +2.08 (0.36)\\
        & T & ASim & \textbf{0.00} (0.01) & \textbf{-0.01} (0.00) &  &  & \textbf{+0.18} (0.04) \\
        \midrule
        \multirow{8}{*}{\rotatebox{90}{BPI17W}} & L & real & 0.54 (0.01) & 0.88 (0.00) & 6.10 (0.55) & 33.01 (0.15) & 6.61 (0.40) \\
        & T & real & 0.62 (0.01) &  & 6.14 (0.26) & 33.23 (0.43) &  \\    
        \cdashline{2-8}
        & L & Simod & -0.23 (0.00) & -0.35 (0.00) & \textbf{-0.56} (0.00) & -0.12 (0.00) & +0.68 (0.00) \\
        & L & DSim & -0.19 (0.02) & NA & +3.46 (3.66) & -0.10 (0.04) & +0.62 (0.06) \\
        & L & ASim & \textbf{-0.08} (0.09) & \textbf{0.00} (0.00) & +1.70 (2.50) & \textbf{0.00} (0.15) & \textbf{+0.25} (0.36) \\      
        & T & Simod & -0.20 (0.00) &  & -0.25 (0.00) & +9.48 (0.00) &  \\
        & T & DSim & -0.29 (0.09) & NA & +0.07 (0.22) & +21.95 (12.02) & \\
        & T & ASim & \textbf{-0.12} (0.14) &  & \textbf{-0.06} (0.08) & \textbf{+9.22} (7.19) &  \\
        \bottomrule
    \end{tabular}
    \label{tab:results_real}
\end{table}
